MetaPoison: Practical General-purpose Clean-label Data Poisoning

Data poisoning -- the process by which an attacker takes control of a model by making imperceptible changes to a subset of the training data -- is an emerging threat in the context of neural networks. Existing attacks for data poisoning neural networks have relied on hand-crafted heuristics, because solving the poisoning problem directly via bilevel optimization is generally thought of as intractable for deep models. We propose MetaPoison, a first-order method that approximates the bilevel problem via meta-learning and crafts poisons that fool neural networks. MetaPoison is effective: it outperforms previous clean-label poisoning methods by a large margin. MetaPoison is robust: poisoned data made for one model transfer to a variety of victim models with unknown training settings and architectures. MetaPoison is general-purpose, it works not only in fine-tuning scenarios, but also for end-to-end training from scratch, which till now hasn't been feasible for clean-label attacks with deep nets. MetaPoison can achieve arbitrary adversary goals -- like using poisons of one class to make a target image don the label of another arbitrarily chosen class. Finally, MetaPoison works in the real-world. We demonstrate for the first time successful data poisoning of models trained on the black-box Google Cloud AutoML API. Code and premade poisons are provided at https://github.com/wronnyhuang/metapoison

==> old_text.tex <==
% \documentclass{article}

% %
% %http://metalearning.ml/2019/#submission-instructions

% % if you need to pass options to natbib, use, e.g.:
% % \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2019

% % ready for submission
% \usepackage[]{neurips_2019}

% % to compile a preprint version, e.g., for submission to arXiv, add
% % add the [preprint] option:
% % \usepackage[preprint]{neurips_2019}

% % to compile a camera-ready version, add the [final] option, e.g.:
% % \usepackage[final]{neurips_2019}

% % to avoid loading the natbib package, add option nonatbib:
% % \usepackage[nonatbib]{nips_2019}

% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage[hidelinks]{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography

% %some packages we added
% \usepackage{hyperref}
% \pdfoutput=1
% % Recommended, but optional, packages for fig and better typesetting:
% \usepackage{graphicx}

% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{natbib}
% \bibliographystyle{unsrtnat}
% \usepackage{subcaption}
% \usepackage{caption}
% \usepackage{placeins}
% \usepackage{wrapfig}

% \usepackage{amsmath}
% \usepackage{xcolor}
% \captionsetup[subfigure]{width=0.95\textwidth}

% \newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}
% \newcommand{\tom}[1]{{  \textcolor{red}{\bf \em [Tom: #1]}}}
% \newcommand{\comment}[1]{{  \textcolor{red}{\bf \em [Tom: ...#1]}}}
% \newcommand{\ronny}[1]{{  \textcolor{blue}{\bf \em [Ronny: #1]}}}
% \newcommand{\liam}[1]{{  \textcolor{purple}{\bf \em [Liam: #1]}}}
% \newcommand{\micah}[1]{{  \textcolor{green}{\bf \em [Micah: #1]}}}
% \newcommand{\fh}[1]{{   \textcolor{red}{\bf \em [Furong: #1]}}}

% \title{Appendix for ``MetaPoison: Learning to Craft Adversarial Poisoning Examples via Meta-Learning''}
% % todo using placeholder, Will revise
% \author{
% W. Ronny Huang\\
% %\thanks{Use footnote for providing further
% %information about author (webpage, alternative
% %address)---\emph{not} for acknowledging funding agencies.} \\
% University of Maryland\\
% \texttt{wrhuang@umd.edu}\\
% %% examples of more authors
% \And
% Zeyad Emam\\
% University of Maryland\\
% \texttt{zeyad@math.umd.edu}\\
% \AND
% Jonas Geiping\\
% University of Siegen\\
% \texttt{jonas.geiping@uni-siegen.de}\\
% \And
% Liam Fowl\\
% University of Maryland\\
% \texttt{lfowl@math.umd.edu}\\
% \And
% Justin K. Terry\\
% University of Maryland\\
% \texttt{justinkterry@gmail.com}\\
% \AND
% % Abhay K. Yadav\\
% % University of Maryland\\
% % \texttt{jaiabhay@cs.umd.edu}\\
% % \And
% Furong Huang\\
% University of Maryland\\
% \texttt{furongh@cs.umd.edu}\\
% \And
% Tom Goldstein\\
% University of Maryland\\
% \texttt{tomg@cs.umd.edu}\\
% }

% \begin{document}

%     \maketitle


% \appendix 


MetaPoison is a versatile paradigm for data poisoning in various threat models. We will focus on several situations and threat models in this experimental section to show this, ranging from finetuning as considered in \citep{shafahi2018poison} to poisoning-from-scratch, which was not feasible before.

\subsection{Experimental Setup}

\subsection{OLDTEXT}
%We perform our training and poison crafting on a subset of CIFAR-10 which contains the first 500 examples from each class. In the appendix we show analogous results for the case of the entire CIFAR-10. We choose the first image in the test set, a ``cat,'' to be the target image, and we choose the first class in the training set, the ``airplane'' class, to be the adversarial label. We allow for a poison budget of $n/N=4\%$, which corresponds to $n=200$ poisons, which are taken to be the first 200 images in the source class. The model architecture is a simple 6-layer convolutional network, akin to the one used in MAML (\cite{finn2017model}).
We test the developed algorithm by considering the task of poisoning a standard Resnet-20 trained on the CIFAR-10 dataset\footnote{All code for these experiments can be found in the (anonymized) github repository at \url{https://github.com/2350532677/metapoison}}. Standard network implementation, training procedure, and data augmentation techniques are used\footnote{Resnet model and training procedure: \url{https://github.com/tensorflow/models/tree/master/official/resnet}}. For our attacks we generally choose a random target image from the CIFAR-10 test set and choose the first $n$ images from a random poison class as the source images.
%In the following we will usually denote this setup by the triplet (\textit{PoisonLabel}-\textit{TargetLabel}-\textit{AdversarialLabel}), denoting from which class we draw images that will contain poison, which class the target image is and which class the intended label is.

We use the typical cross entropy loss as our objective function during poison crafting and make poison updates using the Adam optimizer \cite{carlini2017towards}. We project onto the constraint $\|\Delta\|_\infty < \epsilon$ after each gradient update, with $\epsilon=16/255$. %Figure \ref{fig:cifar-tenth} shows the results of crafting poisons based on an ensemble of $N_{models}=20$ surrogate models. 


Examples for poisoned images can be seen in Figure \ref{fig:images}. Figure \ref{fig:victims_still_work} shows that inserting the poison into training successfully changes the label of the targeted image for nearly 100\% of initializations, without affecting the validation accuracy of the other training images, making the attack imperceptible without knowledge of the target image or detection of the adversarial pattern. 

\subsubsection{Crafting process}
Figure \ref{fig:crafting_process} visualizes the progress of the poison during the crafting phase. The first-order nature of the crafting process is clearly visible in \ref{fig:crafting_process-a}. After unrolling for a few steps, we find that the \textit{unrolled state} target loss $L(x_t, y_\text{source})$ is just slightly lower that of the normal (unaffected) state. Yet, during victim training, these small nudges from the poisons toward lower target loss have a cumulative effect over all training epochs and the target loss decreases significantly, leading to a reclassification of the target image at the end of victim training. Note that each point on the red curve in Figure \ref{fig:crafting_process-a} and dark blue curve in Figure \ref{fig:crafting_process-b} are the target loss and success rate at the end of training when trained from-scratch on the poisons generated \textit{at that particular craft step}. It is further important to note that test accuracy of all other images is only marginally affected, making this attack nearly undetectable, as shown in Figure \ref{fig:crafting_process-b}.
The effectiveness of the poison increases as more information on different network states and examples is accumulated and averaged during the crafting process. 

\subsubsection{Victim training process}
We now take a closer look at what happens when the victim trains their model on the poisoned dataset. One would typically expect that as training progresses, misclassification of the target example (i.e. to the source class or any class other than the target class) will \textit{decrease} as the generalization ability of the model increases. We see in Figure \ref{fig:victims_still_work} that the \textit{adversarial} target loss decreases and attack success rate increases as a function of epoch. Each curve corresponds to a different randomly selected source-target pair and is the average of 8 independent training runs. Further, the test accuracy curve is unaffected. While we train only to 50 epochs here for runtime constraints, the result at 100 epochs almost always the same, since after epoch 40, 60, and 80 in the standard training procedure, the learning rate decreases significantly.

\subsubsection{Effect of poisoning budget}
In Figure \ref{fig:budget} we investigate restrictions into the poison \emph{budget}, that is how many images from the poison class can be accessed during training. For these experiments we use a smaller poison budget. While $10\%$ corresponds to control over the full set of training images from one class, we see that this number can be reduced significantly. The effectiveness varies more between different poison-target pairings, than with the control over the image set. Plainly speaking, an ``easier'' choice for the poison class, is more important than the actual amount of control over it.



\subsubsection{Effect on validation accuracy}
Figure \ref{fig:victims_still_work} and Figure \ref{fig:crafting_process-b} show how small the effect of the poison on the remainder of the validation set really is. While other attacks exist that make training difficult in general or disturb generalization accuracy for all classes, e.g. \cite{steinhardt2017poison}, our method behaves very differently. This is a consequence of the bi-level formulation of the poisoning problem, we minimize the target loss under minimizers of the victim loss. This leads to an almost surgical precision, where precisely only the target image is modified, leaving other images unaffected and making it hard to detect that an attack took place without knowledge of the target image. This is no small feat as the validation set, especially on CIFAR, contains a substantial collection of images similar to the target image.




% \begin{figure}



\subsubsection{Effect on validation accuracy}
Figure \ref{fig:victims_still_work} and Figure \ref{fig:crafting_process-b} show how small the effect of the poison on the remainder of the validation set really is. While other attacks exist that make training difficult in general or disturb generalization accuracy for all classes, e.g. \cite{steinhardt2017poison}, our method behaves very differently. This is a consequence of the bi-level formulation of the poisoning problem, we minimize the target loss under minimizers of the victim loss. This leads to an almost surgical precision, where precisely only the target image is modified, leaving other images unaffected and making it hard to detect that an attack took place without knowledge of the target image. This is no small feat as the validation set, especially on CIFAR, contains a substantial collection of images similar to the target image.



%\subsection{Transferability to different training strategies}
In the threat model considered so far in this investigation, the poisons were investigated on the same architecture and hyper-parameter settings as they were crafted on, so that the only source of difference between training model and victim model was in the initial network parameters. In more general settings, an attacker might be able to reasonably guess the architecture used by the defender, yet the exact hyper-parameters are often unknown. We check the transferability of poisons across hyper-parameters in Figure \ref{fig:transfer}. We find that although there is some variance across different target pairs, the crafted poisons are astonishingly robust against hyperparameter changes. For details, the baseline scenario involves batchsize of 125, learning rate of 0.1, optimizer of Momentum, and no regularization (no data augmentation and weight decay). Corresponding changes in the victim model include: batchsize and learning rate of 250 and 0.2, optimizer of SGD, and regularization which includes weight decay and data augmentation.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{fig/transferplot.png}
%     \caption{Transferrability of poisons developed on one architecture and hyper-parameter setting to a different one. The different columns in each category represent different draws of poison-target class pairings. We see that although ..., the poisons are largely independent of model hyperparameters.}
%     \label{fig:transfer}
% \end{figure}

\subsubsection{Multifaceted attack scenarios}
Beyond the conventional poisoning attack discussed previously, MetaPoison can flexibly attack in other ways. In this section we detail two other attack strategies.\\ %three

\textbf{Third-Party Attack}: 
In this scenario, the attacker has access to just one class of images, e.g. \textit{car}, and wants to transfer a target image of, e.g. \textit{deer} to a ``third-party'' label, e.g. \textit{horse}. If we assume the feature collision discussed in previous works such as \cite{shafahi2018poison} to be a necessary mechanism for clean-label data poisoning, then this attack should be impossible. The features of \textit{car} lie too far away from the features of \textit{horse} to affect the classification of \textit{deer} images. Yet the attack works nearly as well as the default attack, as shown detailed in \ref{fig:attacktypes}.

\textbf{Multi-target attack}:
Previous attacks focused on a single target image. However, an attacker might want to misclassify several target images with the same set of poisons. Interestingly this attack (within the same budget as the single target attack) is relatively difficult. Inter-class variability between different targets makes it difficult for the poisoned images to be effective in all situations and the reliability of the poisoning decreases.

% \textbf{Multi-class poison attack}: 
% Whereas we considered an attack model where the attacker can only modify a budget of images from a single class, we now consider the reverse case: The attacker is allocated a random subset of images from the training set and has to craft a poison with this budget. This threat model leads to a difficult avenue to attack, the poisoning process is not able to stabilize due to variablity in the poison images and the final poisoning is unreliable. %This threat model is furthermore problematic to realize in practice, as an attacker needs to have knowledge of the selection process used to generate the training set?

% \begin{figure}
%     \centering
%     \includegraphics[width=0.32\textwidth]{fig/thirdparty.png}
%     \includegraphics[width=0.32\textwidth]{fig/multitarget.png}
%     \includegraphics[width=0.32\textwidth]{fig/multiclass.png}
%     \caption{Different attack strategies and threat models. Left: Third-Party Attacks. Middle: Attack on multiple targets. Right: Attack with random poison images (from any class). We find that Third-Party attacks (Using the images from the first class to perturb the classification of an image of the second class into the third class) are often quite effective. Increasing the number of targets that can be attack with the same poison budget however is difficult. Even more so is poisoning with images from very unrelated classes that are spread across classes.}
%     \label{fig:attack_scenarios}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}[t]{0.32\textwidth}
%         \centering
%         \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/thirdparty.png}
%         \caption{Third-Party Attacks. (Using the images from the first class to perturb the classification of an image of the second class into the third class) are reasonably effective.\label{fig:thirdparty}}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.32\textwidth}
%         \centering
%         \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/multitarget.png}
%         \caption{Attack on multiple targets from the same class. These attacks are potentiall more difficult as the poisons need to contend with inter-class variability.\label{fig:multitarget}}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.32\textwidth}
%         \centering
%         \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/multiclass.png}
%         \caption{Attack with random poison images (from any class). These attacks are the hardest. When attacker can only modify a small random subset of training images, then most images are possibly not informative enough to construct a strong poison.\label{fig:randompoison}}
%     \end{subfigure}
%     \caption{\small Different attack strategies and threat models. All lines are marked as \textit{Poison-Label}-\textit{Target-Label}-\textit{Intended/Adversarial Label}. \ronny{need to get rid of these figures}}
%      \vspace{-5mm}
%      \label{fig:attack_scenarios}
% \end{figure}

% \begin{wrapfigure}[]{r}
% % \end{figure}
% \end{wrapfigure}



\section{Background}

  In {\em feature collision} attacks, the attacker first chooses a target image whose class label she wishes to alter at test time.  She then makes small perturbations to a training image, called the ``source'' image, so that its feature representation ``collides'' with the feature representation of the target image (\cite{shafahi2018poison}).  During training, the network over-fits on the data, learning to classify the poison source image with its assigned label in the training set.  Then, at test time, the target image has the same feature representation as the poison image, and is assigned the same (but incorrect) label.  Feature collision attacks have been extended to {\em poison polytope} attacks, which work in the black-box setting, and with end-to-end training (\cite{zhu2019transferable}).  However feature collision attacks only work in the case of transfer learning, when a pre-trained model is fine tuned on a small poisoned dataset.  To date, such attacks have not been demonstrated on networks trained from scratch.
{\em Backdoor} attacks insert a pattern or shape into training images that belong to the target class.  The network learns to associate these patterns with the target class, and then mistakenly places images into the target class at test time when they contain that pattern.  Unlike the attacks studied here, backdoor attacks require the attacker to manipulate both train and test inputs.

We are interested in clean-label attacks that only make small perturbations to a subset of training images and leave a normal  ``from scratch'' training procedure otherwise unchanged and unaltered. This type of attack is especially insidious since it is meant to maintain the class label of the poisons, and thus is not susceptible to by-hand data sanitization. 

Meta-learning has gained popularity, particularly as an approach to few-shot learning (\cite{finn2017model,bertinetto2018metalearning,lee2019metalearning}). Often in this setup, training involves an inner loop to take training steps on tasks and an outer loop to back-propagate through these training steps to find optimal network parameters that adapt quickly to new training tasks. We apply a similar framework to poisoning networks below.


\section{Training on entire CIFAR-10 dataset}

We show in Figure \ref{fig:cifar-full} results on training on the entire CIFAR-10 dataset. Due to runtime constraints, we were not able to tune the hyperparameters for this scenario, but the results already show that meta-poisoning is still decently successful, causing up to 70\% success rate at some craft steps.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/craft_cwT,craft_cwT0_50000.jpeg}
        \caption{Carlini-Wagner loss on target example during crafting process. Red: average loss over all unroll steps (crafting objective). Blue: Loss of the target example at the current network weights.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/victim_cwT0_50000.jpeg}
        \caption{Carlini-Wagner loss on target example at the end of 100 steps of victim training, using the poisons at the current craft step (x-axis).}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/victim_accT0_50000.jpeg}
        \caption{Poisoning success rate at the end of 100 steps of victim training using the poisons at the current craft step (x-axis).}
        \label{fig:poison_sucess}
    \end{subfigure}
    \caption{\small Training from scratch with full CIFAR10 training set.}
     \vspace{-5mm}
     \label{fig:cifar-full}
\end{figure}


\section{Computation graph}
In Figure \ref{fig:computation_graph} we show the high-level computation graph for a simple two model ensemble setup to craft the poisons.

\begin{figure}
% \begin{wrapfigure}[]{r}{0.5\textwidth} 
    \centering
    \includegraphics[width=.5\textwidth,trim=0mm 0mm 0mm 0mm]{fig/graph.png}
    \caption{\small High level comptuation graph of our poison crafting scheme. } %APPENDIX???
    % \vspace{-4mm}
    \label{fig:computation_graph}
\end{figure}
% \end{wrapfigure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/plot_one0.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/plot_one1.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=.99\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/plot_one2.png}
        \caption{}
    \end{subfigure}
    \caption{\small Three training curves on clean and poison data with gradients w.r.t. adversarial target loss. PCA performed with 2 components accounting for $96.1$\%, $96.3$\%, and $96.2$\% variance captured for each plot respectively.}
     \vspace{-5mm}
     \label{fig:victims_still_work}
\end{figure}

\section{Reason for applying meta-gradient at the end of the epoch}
\label{sec:epochend}
Rather than updating the perturbations to that mini-batch $\Delta_{i,b}$ right away as in Equation \ref{eq:unroll3}, we store the \textit{partial} meta-gradient $\nabla_{\Delta_b}\mathcal{L}(x_t, y_{adv}; \theta_K)$ (corresponding only to perturbations within that mini-batch) until the current epoch is finished. Then the meta-gradients for all $b$ are concatenated into the \textit{full} meta-gradient and it is then applied to the perturbation $\Delta$. In principle there is no difference whether the batch-wise perturbations are updated immediately or at the end of the epoch for a \textit{single} surrogate model. However, it does matter when we craft with multiple surrogate models and want to average the meta-gradients before updating. In the latter case, we must wait until all the full meta-gradients are available before averaging.



\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=.85\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/craftloss.pdf}
        \caption{Cross entropy loss on the target image after unrolling in \emph{crafting} in comparison to unaffected loss versus actual cross entropy during victim training. Even if the unrolled change is small, the effect on victim training is devastating. The blue and green curves are the losses averaged all our surrogate models (21 here), while the red curve is averaged over multiple victim trainings (4 here). \label{fig:crafting_process-a}} %The first-order nature of the crafting process is clearly visible. After unrolling for a few steps the loss on the target is just slightly lower than the normal (unaffected) state. During victim training, these small unroll steps have a devastating effect and the target loss decreases significantly.}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=.85\textwidth, trim=0cm 0cm 0cm 0cm, clip]{fig/craftacc.pdf}
        \caption{Classification accuracy of the target when training from scratch with the current poison, shown for each step in the crafting procedure. The curves are averaged over 4 independent victim training routines. \label{fig:crafting_process-b}}
    \end{subfigure}
    \caption{\small A look into the process of crafting poisons.}
     %\vspace{-5mm}
     \label{fig:crafting_process}
\end{figure*}


% \bibliography{library}
% \end{document}


